Self-Distillation for Further Pre-training of Transformers

Pre-training a large transformer model on a massive amount of unlabeled data and fine-tuning it on labeled datasets for diverse downstream tasks has proven to be a successful strategy, for a variety of vision and natural language processing tasks. However, direct fine-tuning of the pre-trained model may be suboptimal if there exist large discrepancies across data domains for pre-training and fine-tuning. To tackle this issue, several previous studies have proposed further pre-training strategies, where we continue to pre-train the model on the target unlabeled dataset before fine-tuning. However, all of them solely focus on language models and we empirically find that a Vision Transformer is vulnerable to overfitting as we continue to pretrain the model on target unlabeled data. In order to tackle this limitation, we propose self-distillation as a regularization for a further pre-training stage. Specifically, we first further pre-train the initial pre-trained model on the target unlabeled data and then consider it as a teacher for self-distillation. Then we take the same initial pre-trained model as a student and enforce its hidden representations to be close to those of the teacher while optimizing the student with a masked auto-encoding objective. We empirically validate the efficacy of self-distillation on a variety of benchmark datasets for image and text classification tasks. Experimentally, we show that our proposed method outperforms all the relevant baselines. Theoretically, we analyze the proposed method with a simplified model to understand how self-distillation for further pre-training can potentially help improve the performance of the downstream tasks.

==> figures/low_resource.tex <==
\begin{wrapfigure}{r}{0.36\textwidth}
\vspace{-0.2in}
 \centering
  \includegraphics[width=0.36\textwidth]{images/low_resource_bar.pdf}
  \vspace{-0.3in}
  \caption{\small Accuracy with varying the number of training data.}
  \vspace{-0.1in}
  \label{fig:low-resource}
\end{wrapfigure}





==> figures/multi_round_acc.tex <==
\begin{wrapfigure}{r}{0.35\textwidth}
\vspace{-0.2in}
 \centering
  \includegraphics[width=0.35\textwidth]{images/round_distill.png}
  \vspace{-0.22in}
  \caption{\small Test accuracy as a function of self-distillation round $t$.}
  \vspace{-0.13in}
  \label{fig:multi-round-acc}
\end{wrapfigure}





==> tables/ablation.tex <==
\begin{wrapfigure}{t}{0.4\textwidth}
\small
\centering
\vspace{-0.2in}
\captionof{table}{\small Ablation on CUB and SCIERC.}
\vspace{-0.1in}
\resizebox{0.4\textwidth}{!}{
\begin{tabular}{lcc}
\toprule
\textbf{Model} & \textbf{CUB} & \textbf{SCIERC} \\
\midrule
Full Model & $\textbf{58.06}\pm\textbf{0.90}$ & $\textbf{81.79}\pm\textbf{0.75}$ \\ 
\midrule
w/o $\mathcal{L}_\texttt{MAE}$ & $57.60\pm0.81$ & $80.66\pm0.62$ \\
w/o $\mathcal{L}_\texttt{Distill}$ & $55.72\pm{0.46}$ & $80.32\pm1.25$ \\
Further Pre-train$\times2$ & $53.41\pm0.75$ & $80.52\pm0.98$ \\
Prediction-Matching &  $55.27\pm1.07$ & $81.09\pm1.07 $\\
Weight-Matching ($\ell_2$)  & $53.70\pm0.91$ & $80.54\pm1.21$\\
Weight-Matching (MARS) & $54.82\pm0.60$ & $80.95\pm0.71$\\ 
\bottomrule
\end{tabular}
}
\vspace{-0.1in}
\label{tab:ablation}
\end{wrapfigure}
